A Measure Theoretic Proof of $\mathfrak p=\mathfrak t$

Rothberger's question of whether the two cardinals $\mathfrak p$ and $\mathfrak t$ are equal, posed back in 1948, was only answered fairly recently in the affirmative. Here we answer the more difficult progenitor question (posed in the same place) on when filter-bases can be refined to towers. Of equal import, our proof that $\mathfrak p=\mathfrak t$ addresses issues raised by Gowers concerning the "proof path" of the original solution. This is applied to obtain a gap spectrum result for the ultrapowers $\mathbb N^{\mathbb N}\,/\,{\mathcal U}$.

==> macros.tex <==

\makeatletter
% macros:

% axioms

\newcommand{\ch}{\mathrm{CH}}
\newcommand{\gch}{\mathrm{GCH}}
\newcommand{\ma}{\mathrm{MA}}
\newcommand{\map}{\ma^+}
\newcommand{\zfc}{\mathrm{ZFC}}
\newcommand{\zfcf}{\mathrm{ZFC}^*}
\newcommand{\zfcm}{\mathrm{ZFC}^-}
\newcommand{\zf}{{\mathrm{ZF}}}
\newcommand{\ac}{\mathrm{AC}}
\newcommand{\zfm}{\mathrm{ZF}^-}
\newcommand{\pfa}{\mathrm{PFA}}
\newcommand{\mm}{\mathrm{MM}}
\newcommand{\rvm}{\mathrm{RVM}}
\newcommand{\vhod}{V\mathop{=}\hod}
\newcommand{\oca}{\operatorname{OCA}}
\newcommand{\Paxiom}{\mathrm{P}}

% combinatorial principles

\newcommand{\sm}{\textrm{\rm SM}}
\newcommand{\sh}{\textrm{\rm SH}}
\newcommand{\kh}{\mathrm{KH}}
\newcommand{\pstar}{(*)}
\newcommand{\pstarc}{(\gdot_c)}
\newcommand{\pstarcm}{(\gdot_c^-)}
\newcommand{\pstarcmm}{(\gdot_c^{=})}
\newcommand{\pstarcp}{(\gdot_c^+)}
\newcommand{\pstarfalse}{\text{(\ding{75})}}
\newcommand{\rsh}{\mathrm{RSH}}
\newcommand{\rkh}{\mathrm{RKH}}

% operators

%% unary

\newcommand{\dom}{\operatorname{dom}}
\newcommand{\ran}{\operatorname{ran}}
\newcommand{\proj}{\operatorname{proj}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\Lim}{\operatorname{Lim}}
\newcommand{\dense}{\operatorname{Dense}}
\newcommand{\game}{\Game}
\newcommand{\deriv}{\partial}
\newcommand{\spn}{\operatorname{span}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\length}{\operatorname{len}}
\newcommand{\rep}{\operatorname{rep}}
\newcommand{\downcl}[1]{{\downarrow\hspace{-2.5pt}#1}}
\newcommand{\upcl}[1]{{\uparrow\hspace{-2.5pt}#1}}
\newcommand{\interior}{^\circ}
\newcommand{\ro}{\operatorname{RO}}
\newcommand{\gdot}{\star}
\newcommand{\power}{\P}
\newcommand{\lbrak}{\bigl\|}
\newcommand{\rbrak}{\bigr\|}
\newcommand{\lmeas}{\mu\bigl(\lbrak}
\newcommand{\rmeas}{\rbrak\bigr)}
%\newcommand{\e}[1]{^{[#1]}}
\newcommand{\inv}{^{-1}}
\newcommand{\bigsetminus}{\mathbin{\big\backslash}}
\newcommand{\powfin}[1]{[#1]^{<\aleph_0}}
\newcommand{\powcnt}[1]{[#1]^{\leq\aleph_0}}
\newcommand{\powcif}[1]{[#1]^{\aleph_0}}
\newcommand{\powinf}{\power_{\!\infty}}
%\newcommand{\powfin}{\power_{\fin}}
\newcommand{\coh}{\operatorname{Cohen}}
\newcommand{\rand}{\operatorname{Random}}
\newcommand{\cf}{\operatorname{cf}}
\newcommand{\otp}{\operatorname{otp}}
\newcommand{\pred}{\operatorname{pred}}
\newcommand{\hit}{\operatorname{ht}}
\newcommand{\ext}{^\smallfrown\hspb}
\newcommand\bigext{^\frown}
%\newcommand{\crit}{\operatorname{crit}}
\newcommand{\djun}{\amalg}
\newcommand{\lands}{\mathrel{\land}}
\newcommand{\lors}{\mathrel{\lor}}
\renewcommand{\div}{\mathbin{/}}
\newcommand{\cond}{\mathbin{|}}
\newcommand{\bigcond}{\mathbin{\big|}}
\newcommand{\Bigcond}{\mathbin{\Big|}}
\newcommand{\Biggcond}{\mathbin{\Bigg|}}
\newcommand{\diff}{\operatornamewithlimits{\bigtriangleup}}
\newcommand{\Ex}{\operatorname{E}}
\newcommand{\con}{\operatorname{Con}}
\renewcommand{\succ}{\operatorname{succ}}
\newcommand{\imsucc}{\operatorname{imsucc}}
\newcommand{\symdiff}{\bigtriangleup}
\newcommand{\clopen}{\operatorname{Clopen}}
\newcommand{\borel}{\operatorname{Borel}}
\newcommand{\cat}{\operatorname{Cat}}
\newcommand{\cts}{C}
%\newcommand{\alg}{\operatorname{alg}}
\newcommand{\Gen}{\operatorname{Gen}}
\newcommand{\Genc}{\operatorname{Gen}^+}
\newcommand{\Ult}{\operatorname{Ult}}
\newcommand{\pfn}{\dashrightarrow}
\newcommand{\elspc}[1]{\ell^{#1}}
\newcommand{\inj}{\operatorname{inj}}
\newcommand{\ds}[1]{\O_{#1}}
\newcommand{\id}{\operatornamewithlimits{id}}
\newcommand{\gid}{e}
\newcommand{\funct}{\operatorname{Fnct}}
\renewcommand{\hom}{\operatorname{Hom}}
\newcommand{\edo}{\operatorname{Endo}}
\newcommand{\mono}{\operatorname{Mono}}
\newcommand{\smono}{\underleftarrow{\mono}}
\newcommand{\epi}{\operatorname{Epi}}
\newcommand{\sepi}{\underleftarrow{\vspace{-1.5pt}\epi}}
\newcommand{\aut}{\operatorname{Aut}}
\newcommand{\preiso}{\operatorname{Preiso}}
\newcommand{\iso}{\operatorname{Iso}}
\newcommand{\act}{\operatorname{Act}}
\newcommand{\pos}{\operatorname{pv}}
\newcommand{\atom}{\operatorname{At}}
\newcommand{\sym}{\operatorname{sym}}
\newcommand{\modty}{\operatorname{mod}}

%%% shadows/shades

\newcommand{\@shade}[2]{\nabla_{#1#2}}
\newcommand{\@shadow}[2]{\Delta_{#1#2}}
\newcommand{\shadeto}[1]{\@shade{\to}{#1}}
\newcommand{\shadowto}[1]{\@shadow{\to}{#1}}

% meant to be used as infimum and supremum
\newcommand{\ifm}{\bigwedge}
\newcommand{\spr}{\bigvee}

%% binary operators

\newcommand{\lorand}{{\lor}\hspace{-4pt}{\land}}

\newcommand{\altrstr}{\mathbin{\upharpoonleft}}
\providecommand{\restriction}{\mathbin{\upharpoonright}}
\newcommand{\dual}[1]{\bigl(#1\bigr)^*}
\newcommand{\coprd}{\mathop{\oplus}}

\newcommand{\iprod}[2]{\<#1,#2\>}


% relations

\newcommand{\compat}{\approx}
\newcommand{\incompat}{\not\approx}
\newcommand{\rel}{\mathrel{R}}
\newcommand{\subgp}{\leqdot}
\newcommand{\precle}{\preccurlyeq}

%% templates for enhanced relations

\newcommand{\@@eq}[2]{=_{#1}^{#2}}
\newcommand{\@@neq}[2]{\ne_{#1}^{#2}}
\newcommand{\@@l}[2]{<_{#1}^{#2}}
\newcommand{\@@nl}[2]{\nless_{#1}^{#2}}
\newcommand{\@@le}[2]{\le_{#1}^{#2}}
\newcommand{\@@nle}[2]{\nleq_{#1}^{#2}}
\newcommand{\@@equiv}[2]{\equiv_{#1}^{#2}}

\newcommand{\@in}[1]{\in_#1}
\newcommand{\@eq}[1]{=_#1}
\newcommand{\@le}[1]{\le_{#1}}
\newcommand{\@l}[1]{<_#1}
\newcommand{\@nle}[1]{\nleq_#1}
\newcommand{\@ge}[1]{\ge_#1}

\newcommand{\u@le}[1]{\le^#1}
\newcommand{\u@l}[1]{<^#1}
\newcommand{\u@eq}[1]{=^#1}

\newcommand{\@lefnt}[1]{\@@le#1*}
\newcommand{\@nlefnt}[1]{\@@nle#1*}
\newcommand{\@eqfnt}[1]{\@@eq#1*}

\newcommand{\@supseteq}[1]{\supseteq_{#1}}
\newcommand{\@subseteq}[1]{\subseteq_{#1}}
\newcommand{\@nsubseteq}[1]{\nsubseteq_{#1}}

%% quotient relations

\newcommand{\qle}[1]{{\le}\div#1}

%% standard enhanced

\newcommand{\subseteqfnt}{\subseteq^*}
\newcommand{\subsetfnt}{\mathrel{\subset^*}}
\newcommand{\nsubseteqfnt}{\mathrel{\nsubseteq^*}}
\newcommand{\supseteqfnt}{\mathrel{\supseteq^*}}
\newcommand{\supsetfnt}{\mathrel{\supset^*}}
\newcommand{\lefnt}{\mathrel{\le^*}}
\newcommand{\nlefnt}{\nleq^*}
\newcommand{\lneqfnt}{\lneq^*}
\newcommand{\gefnt}{\mathrel{\ge^*}}
\newcommand{\ngefnt}{\ngeq^{*}}
\newcommand{\eqfnt}{\mathrel{=^*}}
\newcommand{\neqfnt}{\mathrel{\ne^*}}
\newcommand{\lfnt}{<^*}
\newcommand{\nlfnt}{\nless^*}
\newcommand{\gfnt}{>^{*}}
\newcommand{\ngfnt}{\ngtr^{*}}
\newcommand{\laux}{\lessdot^{*}}
\newcommand{\nlaux}{\not\mathrel{\lessdot}^{*}}
\newcommand{\dle}{\mathrel{\dot\le}}
\newcommand{\dperp}{\mathrel{\dot\perp}}
\newcommand{\proves}{\vdash}
%\newcommand{\divides}{\mathrel{|}}
\newcommand{\len}[1]{\@le{#1}}
\newcommand{\lln}[1]{\@l#1}
\newcommand{\gen}[1]{\@ge{{#1}}}
\newcommand{\altle}{\lesssim}
\newcommand{\altl}{\lnsim}
\newcommand{\naltle}{\not\altle}
\newcommand{\altaltle}{\sqsubseteq}
\newcommand{\naltaltle}{\not\sqsubseteq}
\newcommand{\altaltless}{\sqsubset}
\newcommand{\naltaltless}{\not\sqsubset}
\newcommand{\refinefnt}{\mathrel{\preccurlyeq^{*}}}
\newcommand{\rrefinefnt}{\mathrel{\succcurlyeq^*}}
\newcommand{\ld}{<_{\mathrm{d}}}
\newcommand{\ltwo}{<^2}
\newcommand{\letwo}{\le^2}
\newcommand{\linfty}{<^\infty}
\newcommand{\lla}{<_{L[a]}}
\newcommand{\divrel}[2]{\mathrel{{#1}\div{#2}}}
\newcommand{\supseteqn}[1]{\@supseteq{#1}}
\newcommand{\subseteqn}[1]{\@subseteq{#1}}
\newcommand{\nsubseteqn}[1]{\@nsubseteq{#1}}     

%% augmented relations

\newcommand{\str}{\mathrm{str}}
\newcommand{\sep}{\mathrm{sep}}
\newcommand{\asym}{\mathrm{asym}}
\newcommand{\trn}{\mathrm{tran}}
\newcommand{\negstr}{-\str}

\newcommand{\epio}{\preccurlyeq}
\newcommand{\linlen}[1]{\le_{#1}^{\mathrm{lin}}}
\newcommand{\nlinlen}[1]{\nleq_{#1}^{\mathrm{lin}}}
\newcommand{\linln}[1]{<_{#1}^{\mathrm{lin}}}
\newcommand{\ggen}[1]{\gg_{#1}}
\newcommand{\slinlen}[1]{\le_{#1}^{\mathrm{slin}}}
\newcommand{\nslinlen}[1]{\nleq_{#1}^{\mathrm{slin}}}
\newcommand{\strlen}[1]{\@@le{#1}\str}
\newcommand{\nstrlen}[1]{\@@nle{#1}\str}
\newcommand{\strln}[1]{\@@l{#1}\str}
\newcommand{\nstrln}[1]{\@@nl{#1}\str}
\newcommand{\strequiv}[1]{\@@equiv{#1}\str}
\newcommand{\corlen}[1]{\le_{#1}^{\mathrm{cor}}}
\newcommand{\ncorlen}[1]{\nleq_{#1}^{\mathrm{cor}}}
\newcommand{\seple}{\le^\sep}
\newcommand{\lenn}[2]{\@@le{#1}{#2}}
\newcommand{\nlenn}[2]{\@@nle{#1}{#2}}
\newcommand{\lnn}[2]{\@@l{#1}{#2}}
\newcommand{\nlnn}[2]{\@@nl{#1}{#2}}
\newcommand{\nlen}[1]{\nleq_{#1}}
\newcommand{\lneqn}[1]{\lneq_{#1}}
\newcommand{\leu}[1]{\le^{#1}}
\newcommand{\nleu}[1]{\nleq^{#1}}
\newcommand{\gu}[1]{>^{#1}}
\newcommand{\eqnn}[2]{\@@eq{#1}{#2}}
\newcommand{\neqnn}[2]{\@@neq{#1}{#2}}
\newcommand{\asymle}{\u@le\asym}
\newcommand{\asyml}{\u@l\asym}
\newcommand{\llfnt}{\ll^{*}}
\newcommand{\llenn}[2]{\ll_{#2}^{#1}}
\newcommand{\llen}[1]{\ll_{#1}}
\newcommand{\strtrnlen}[1]{\@@le{#1}{\str,\trn}}
\newcommand{\strtrnln}[1]{\@@l{#1}{\str,\trn}}
\newcommand{\trnle}{\u@le{\trn}}
\newcommand{\trnl}{\u@l{\trn}}
\newcommand{\trneq}{\u@eq{\trn}}
\newcommand{\negstrlen}[1]{\@@le{#1}\negstr}
\newcommand{\nnegstrlen}[1]{\@@nle{#1}\negstr}
\newcommand{\nnegstrln}[1]{\@@nl{#1}\negstr}
\newcommand{\negstreq}[1]{\@@eq{#1}\negstr}
\newcommand{\altaltlen}[1]{\altaltle_{#1}}


%% ``almost everywhere'' type relations


%% aa relations

\renewcommand{\aa}{\mathrm{aa}}
\newcommand{\eqaa}{\@eq\aa}
\newcommand{\inaa}{\@in\aa}
\newcommand{\laa}{<_\aa}
\newcommand{\leaa}{\@le\aa}
\newcommand{\nleaa}{\@nle\aa}
\newcommand{\geaa}{\@ge\aa}
\newcommand{\lefntaa}{\@lefnt\aa}
\newcommand{\nlefntaa}{\@nlefnt\aa}
\newcommand{\eqfntaa}{\@eqfnt\aa}
\newcommand{\subseteqaa}{\subseteq_{\aa}}
\newcommand{\subseteqfntaa}{\subseteqfnt_{\aa}}
\newcommand{\lfntaa}{\lfnt_{\aa}}
\newcommand{\relaa}{\rel_{\aa}}

\newcommand{\subseteqfntae}{\subseteq_{\ae}}

%% naa relations

\newcommand{\naa}{\mathrm{naa}}
\newcommand{\eqnaa}{\@eq\naa}
\newcommand{\eqfntnaa}{\@eqfnt\naa}
\newcommand{\lenaa}{\@le\naa}
\newcommand{\lefntnaa}{\@lefnt\naa}
\newcommand{\lfntnaa}{\lfnt_{\naa}}
\newcommand{\nlfntaa}{\nless_{\aa}^{*}}

%% ae relations

\newcommand{\eqae}{\@eq\ae}
\newcommand{\leae}{\@le\ae}

%% fix ??

\newcommand{\subseteqnwd}{\subseteq_{\mathrm{nwd}}}

% Fix This!
\newcommand{\forces}{\mskip 5mu plus 5mu\|\hspace{-2.5pt}{\textstyle \frac{\hspace{4.5pt}}{\hspace{4.5pt}}}\mskip 5mu plus 5mu}

% Logical, spelled out

\newcommand{\Iff}{\espc\mathrm{iff}\espc}
\newcommand{\If}{\espc\textrm{if}\espc}
\newcommand{\impls}{\espc\mathrm{implies}\espc}
\newcommand{\imply}{\espc\mathrm{imply}\espc}
\providecommand{\And}{\espc\mathrm{and}\espc}
\newcommand{\hAnd}{\mathrm{and}\espc}
\renewcommand{\and}{\hespc\mathrm{and}\hespc}
\newcommand{\hand}{\mathrm{and}\hespc}
\newcommand{\OR}{\espc\mathrm{or}\espc}
\newcommand{\hOR}{\mathrm{or}\espc}
\newcommand{\Or}{\hespc\mathrm{or}\hespc}
\newcommand{\hOr}{\mathrm{or}\hespc}

\renewcommand{\iff}{\leftrightarrow}

% cardinal invariants

\renewcommand{\a}{\mathfrak a}
\renewcommand{\b}{\mathfrak b}
\renewcommand{\d}{\mathfrak d}
\newcommand{\cntum}{\mathfrak c}
\newcommand{\f}{\mathfrak f}
\newcommand{\h}{\mathfrak h}
\renewcommand{\i}{\mathfrak i}
\newcommand{\lr}{\mathfrak l\mathfrak r}
\newcommand{\m}{\mathfrak m}
\newcommand{\p}{\mathfrak p}
\renewcommand{\t}{\mathfrak t}
\renewcommand{\r}{\mathfrak r}
\newcommand{\s}{\mathfrak s}
\newcommand{\se}{\mathfrak s\mathfrak e}
\renewcommand{\u}{\mathfrak u}
\newcommand{\x}{\mathfrak x}
\newcommand{\z}{\mathfrak z}

\newcommand{\add}{\operatorname{add}}
\newcommand{\cov}{\operatorname{cov}}
\newcommand{\non}{\operatorname{non}}
\newcommand{\cof}{\operatorname{cof}}

% sets

\newcommand{\two}{\{0,1\}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\Fin}{\mathrm{Fin}}
\newcommand{\pN}{\power(\N)}
\newcommand{\reals}{\mathbb R}
\newcommand{\complex}{\mathbb C}
\newcommand{\N}{\mathbb N}
\newcommand{\pQ}{\power(\rational)}
\newcommand{\Nwd}{\mathrm{Nwd}}
\newcommand{\even}{\mathrm{even}}
\newcommand{\odd}{\mathrm{odd}}
\newcommand{\integers}{\mathbb Z}
\newcommand{\rationals}{\mathbb Q}
\newcommand{\field}{\mathbb F}
\newcommand{\dyadic}{\rationals_{\hsp\mathrm{d}}}
%\newcommand{\irrationals}{\N^{[\infty]}}
\newcommand{\irrational}{\irrationals}

%% sequences

\newcommand{\cantor}{\two^{\hsp\mathbb N}}
\newcommand{\cantorcube}[1]{\two^{\hsp#1}}
\newcommand{\irrationals}{\mathbb N^{\hsp\mathbb N}}
\newcommand{\irri}[1]{\N^{\hsp#1}}
\newcommand{\fintree}{\N^{[<\infty]}}
\newcommand{\fintreeseq}{(\N^{[<\infty]})^\N}
\newcommand{\baireup}{\N_{\scriptscriptstyle\nearrow}^{\hsp\N}}
\newcommand{\irrup}{\irr_{\scriptscriptstyle\nearrow}}
\newcommand{\irrinj}{\N^{\hsp\N}_{\scriptscriptstyle\righttoleftarrow}}
\newcommand{\twoseq}{\two^{<\mathbb N}}
\newcommand{\finseq}{\N^{<\N}}
\newcommand{\bsg}{\intgr^{\N}}
\newcommand{\seq}[1]{{#1}^{<\N}}

\newcommand{\nulls}{\mathcal N}
\newcommand{\meager}{\M}
\newcommand{\meagerp}{\meager^+}
\newcommand{\bp}{\mathrm{BP}}
\newcommand{\fin}{\mathrm{fin}}
\newcommand{\finp}{\Fin^{+}}
\newcommand{\FIN}{\mathrm{FIN}}
\newcommand{\NS}{\mathcal{NS}}
\newcommand{\powerup}[2]{#1_{\scriptscriptstyle\nearrow}^{\hsp#2}}
\newcommand{\ord}{\mathrm{On}}
\newcommand{\hod}{\mathrm{HOD}}
\newcommand{\pnfin}{\pN\div\Fin}
\newcommand{\irrfin}{\irr\div\Fin}
\newcommand{\cohen}{\C}
%\newcommand{\sqideal}{\ideal_{\square}}
\newcommand{\cideal}{\ideal_{\svector C}}
\newcommand{\mak}{\R}
\newcommand{\random}{\R}
\newcommand{\collapse}{\C\O}
\newcommand{\coll}{\mathrm{Col}}
\newcommand{\ctbl}{{\C}{\T}}
\newcommand{\point}{{\perp}}
\newcommand{\pmax}{\mathbb P_{\mathrm{max}}}

%% Borel versions

\newcommand{\borelaa}[1]{\borel(#1)\div{\eqaa}}

%% Baire versions

\newcommand{\baire}{\operatorname{Baire}}
\newcommand{\bfin}{\baire(\Fin)}
\newcommand{\bfinp}{\baire(\finp)}
\newcommand{\birr}{\baire(\irr)}
\newcommand{\birraa}{\birr\div{\eqaa}}
\newcommand{\baireaa}[1]{\baire(#1)\div{\eqaa}}
\newcommand{\bpn}{\baire(\pN)}
\newcommand{\bsirr}[1]{\baire(#1,\irr)}


%% Categories

\newcommand{\cabs}{\mathbf{C}}
\newcommand{\relc}{\mathbf{Rel}}
\newcommand{\qo}{\mathbf{Q}}
\newcommand{\po}{\mathbf{P}}
\newcommand{\lat}{\mathbf{Lat}}
\newcommand{\ql}{\mathbf{QL}}
\newcommand{\ba}{\mathbf{BA}}
\newcommand{\dcpo}{\mathbf{DCPO}}
\newcommand{\clt}{\mathbf{CLT}}
\newcommand{\mgm}{\mathbf{Mag}}
\newcommand{\mon}{\mathbf{Mon}}
\newcommand{\grp}{\mathbf{Grp}}

% ornaments

% Fix all this:
\DeclareFontFamily{U}{cmsy}{}
\DeclareFontShape{U}{cmsy}{m}{n}{<12> sfixed * [10] cmsy10 
<10> <9> <8> <7> <6> <5> sfixed * [10] cmsy10}{}
\DeclareSymbolFont{customtwo}{U}{cmsy}{m}{n} 
\DeclareMathSymbol{\sctn}{\mathord}{customtwo}{"78}

\DeclareFontFamily{U}{cmmi}{}
\DeclareFontShape{U}{cmmi}{m}{n}{<20> sfixed * [11] cmmib10 <12> sfixed * [10]
cmmi10 <10> <9> <8> sfixed * [6] cmmi6 <5> <6> <7> sfixed * [5] cmmi5}{}
\DeclareSymbolFont{custom}{U}{cmmi}{m}{n}
\DeclareMathSymbol{\rharpoon}{\mathord}{custom}{"2A}
%\renewcommand{\vector}{\overset{\raisebox{-1.7pt}[0cm][0cm]{$\rharpoon$}}}
\newlength{\widt}
\newlength{\widttwo}
\newlength{\hgt}
\renewcommand{\vector}[1]{\settowidth{\widttwo}{$\rharpoon$}\addtolength{\widttwo}{-1.0pt}\settowidth{\widt}{$#1$}\settoheight{\hgt}{$#1$}{#1}\hspace{-\widt}\raisebox{\hgt}{$\rharpoon$}\addtolength{\widt}{-\widttwo}\hspace{\widt}}

\newcommand{\svector}[1]{\settowidth{\widttwo}{$\scriptstyle\rharpoon$}\addtolength{\widttwo}{-1.0pt}\settowidth{\widt}{$\scriptstyle#1$}\settoheight{\hgt}{$\scriptstyle#1$}{\scriptstyle#1}\hspace{-\widt}\raisebox{\hgt}{$\scriptstyle\rharpoon$}\addtolength{\widt}{-\widttwo}\hspace{\widt}}
%\renewcommand{\vector}{\vec}

\newcommand{\av}[1]{\settowidth{\widttwo}{$\rharpoon$}\addtolength{\widttwo}{-1.0pt}\settowidth{\widt}{$#1$}\addtolength{\widt}{-1.0pt}\settoheight{\hgt}{$#1$}{#1}\hspace{-\widt}\raisebox{\hgt}{$\rharpoon$}\addtolength{\widt}{-\widttwo}\hspace{\widt}}

% abbreviations

\newcommand{\oone}{{\omega_1}}
\newcommand{\vomega}{\varOmega}
\newcommand{\vlambda}{\varLambda}
\newcommand{\vgamma}{\varGamma}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\real}{\reals}
\newcommand{\irr}{\irrationals}
\newcommand{\rational}{\rationals}
\newcommand{\intgr}{\mathbb{Z}}
\newcommand{\espc}{\quad}
\newlength{\@@hespc}
%\settowidth{\@@hespc}{\quad}
%\setlength{\@@hespc}{\@@hespc/2}
\newcommand{\hespc}{\hspace{\@@hespc}}
\newcommand{\overbar}[1]{\,\overline{\!{#1}}}
%\newcommand{\overbarc}[1]{\
\newcommand{\overbars}[1]{\,\overline{\!{#1}\!}\,}
\newcommand{\overbarg}[1]{\hsp\overline{\hspb{#1}}}
\newcommand{\Th}{{^{\mathrm{th}}}}
\newcommand{\der}[1]{\,\mathrm{d}#1}
\renewcommand{\ae}{\mathrm{ae}}
%\newcommand{\comma}{\text{, }}
\newcommand{\lomega}{L_\omega}
\newcommand{\ul}{\underline}
\newcommand{\ulc}{\ulcorner}
\newcommand{\urc}{\urcorner}
\newcommand{\Bs}{\boldsymbol}
\newcommand{\newent}{\textbf{)\spc(}}
\newcommand{\rcc}{\mathrm{rcc}}
\newcommand{\propk}{\mathrm{property\ }K}
\newcommand{\weakstar}{weak$^*$\ }
\newcommand{\fsto}{\ding{71}}
\newcommand{\tu}{\textup}
\newcommand{\ih}[1]{(\mathrm{IH}_{#1})}

% script letters

\newcommand{\A}{\mathcal A}
\newcommand{\B}{\mathcal B}
\newcommand{\C}{\mathcal C}
\newcommand{\D}{\mathcal D}
\newcommand{\E}{\mathcal E}
\newcommand{\F}{\mathcal F}
%\newcommand{\H}{\mathcal H}
\newcommand{\G}{\mathcal G}
\newcommand{\Hcal}{\mathcal H}
\newcommand{\ideal}{\I}
\renewcommand{\I}{\mathcal I}
\newcommand{\J}{\mathcal J}
\newcommand{\K}{\mathcal K}
\renewcommand{\L}{\mathcal L} % interferes with \L special text character
\newcommand{\M}{\mathcal M}
\newcommand{\Ncal}{\mathcal N}
\renewcommand{\O}{\mathcal O}
\renewcommand{\P}{\Pcal}
\newcommand{\Pcal}{\mathcal P}
\newcommand{\Q}{\mathcal Q}
\newcommand{\R}{\mathcal R}
%\newcommand{\Section}{{\char'237}}
\newcommand{\Scal}{\mathcal S}
\newcommand{\T}{\mathcal T}
\newcommand{\U}{\mathcal U}
\newcommand{\V}{\mathcal V}
\newcommand{\W}{\mathcal W}
\newcommand{\X}{\mathcal X}
\newcommand{\Y}{\mathcal Y}
\newcommand{\Z}{\mathcal Z}

% bb letters

\newcommand{\Ab}{\mathbb A}
\newcommand{\Cb}{\mathbb C}
\newcommand{\Db}{\mathbb D}
\newcommand{\Eb}{\mathbb E}
\newcommand{\Fb}{\mathbb F}
\newcommand{\Gb}{\mathbb G}
\newcommand{\Pb}{\mathbb P}
\newcommand{\Tb}{\mathbb T}
\newcommand{\Qb}{\mathbb Q}

% Frakfurt letters

\newcommand{\Afrak}{\mathfrak A}
\newcommand{\Dfrak}{\mathfrak D}
\newcommand{\Efrak}{\mathfrak E}
\newcommand{\Gfrak}{\mathfrak G}
\newcommand{\Ifrak}{\mathfrak I}
\newcommand{\Mfrak}{\mathfrak M}
\newcommand{\Rfrak}{\mathfrak R}
\newcommand{\Ufrak}{\mathfrak U}

% old script

\newcommand{\Gscr}{\mathscr G}

% spacing

\newcommand{\hsp}{\mspace{1.5mu}}
\newcommand{\hspb}{\mspace{-1.5mu}}
\newcommand{\spc}{\,\,\,}

% LaTeX controls

\newcounter{saveenumi}
\newcommand{\save}{\setcounter{saveenumi}{\value{enumi}}}
\newcommand{\restore}{\setcounter{enumi}{\value{saveenumi}}}
\newcommand{\aref}[1]{{\normalfont(\thechapter.\ref{#1})}}

% toc macros

\newcommand{\addcontentsspace}{\addtocontents{toc}{\protect\vspace{2ex}}}

% index macros

\newcommand{\Index}[1]{#1\index{#1}}
\newcommand{\Dindex}[1]{\emph{#1}\index{#1|emph}}
\newcommand{\Sindex}[1]{#1\index[sym]{#1}}

%% end of macros

